How to Build Digital Humans? From Priors to Photorealistic Avatars

This state-of-the-art report provides an overview of controllable 3D human avatar creation. We describe current 3D avatar systems, which typically consist of three stages: (i) learning priors of human appearance and motion, (ii) creating a personalized avatar, and (iii) animating the avatar. To limit the scope, we focus on the prior learning and avatar creation stages. We define current avatar representations and introduce a taxonomy that categorizes existing work along multiple axes, including body regions and employed priors. We review methods for full-body and head avatars, as well as layered representations that decompose the body into components such as hands, hair, and garments. Finally, we outline common underlying principles, reference key literature for newcomers, and discuss open challenges and future research directions.

==> chapters/2_scope.tex <==
\section{Scope}
\label{sec:scope}

%======================================================================

In this state-of-the-art report, we focus on the various methods for building digital humans. 
%
Specifically, we assume that the motion of the avatar and the camera parameters are given, and concentrate on techniques for photorealistic appearance modeling and synthesis. 
%
%Following the nomenclature introduced by Meta's codec avatars, which distinguishes between the encoder and decoder components of the avatar pipeline \cite{Lombardi21mvp, Saito2024relightable, Bagautdinov2021driving}, this report focuses exclusively on the decoder part. In other words, we study methods that decode control parameters into a digital avatar that is indistinguishable from reality. We explicitly separate our scope from approaches that model motion, such as speech-driven animation \cite{Ng2022learninglisten, Ng2024audio}, path planning, and scene interaction \cite{Tevet2024closd, Dwivedi2025interactvlm, Li2024unimotion, Petrovich2023tmr}, tracking \cite{Zollhofer2018state, Thies2016face}, or geometry reconstruction \cite{Beeler2010highsingle, Beeler2011highpassive}.
%
Our main goal is to develop a practical taxonomy for the field of digital avatars, which will be especially useful not only for people considering work in this area but also for experts already active in the field.
%
This report covers both full-body avatars and individual components such as faces, hair, hands, and garments.
%
We emphasize topics related to building universal priors for avatars and analyze different representations used for tasks in both 2D and 3D. 
%

In \Cref{sec:fundamentals}, we introduce the fundamental components employed by modern methods to build prior models that can generalize across multiple actors, leveraging generative frameworks and statistical analysis.
%
In \Cref{sec:heads,sec:body}, the main chapters, the state-of-the-art methods are presented in detail.
%
We summarize the report with a discussion on challenging aspects of digital avatars, including the cost of avatar generation, and write about future directions and topics.
%

%======================================================================

\subsection{Selection scheme}
As stated above, this report focuses primarily on the appearance of digital avatars. It reviews papers published in the proceedings of major computer vision and computer graphics conferences from 2021 to 2025, as well as preprints available on arXiv. The papers were carefully selected by the authors to fit the scope of this survey and to provide readers with an overview of a broad range of techniques.

This report aims to provide a comprehensive overview of the field, list key literature for those seeking to familiarize themselves with specific research areas, and help standardize notations and definitions. While it covers a diverse selection of recent works, the authors do not claim completeness and strongly encourage readers to consult the cited publications for deeper insights.

%======================================================================

\subsection{Related state-of-the-art reports}
%
\TODO{how are we different from those? -- this is an important section!!}
%
\begin{itemize}
    \item Tracking STAR~\cite{Zollhofer2018state}
    \item 3DMM STAR~\cite{Egger20203d}
    \item Neural Rendering STAR 1~\cite{Tewari2020state}
    \item Neural Rendering STAR 2~\cite{Tewari2022advances}
    \item 3D Face Reconstruction~\cite{Morales2021survey}
    \item Controllable Video Generation~\cite{Ma2025diff_star}
    \item Diffusion Models for Visual Computing~\cite{po2024state}
    \item A Survey on 3D Human Avatar Modeling~\cite{wang2024survey}
    \item 3D human avatar reconstruction with neural fields~\cite{gu20253d}
\end{itemize}

==> chapters/5_6_vol_video.tex <==
\subsection{Volumetric videos}
\label{sec:vol_video}

Sparse view reconstructions/real-time.


==> chapters/6_datasets.tex <==
\section{Datasets}
\label{sec:datasets}

\TODO{here we want to give examples of the datasets used, how they are captured or generated
is it somehow possible to classify how hard it is to get such datasets?
}

Explain how this dataset as captured.

Multiface~\cite{Wuu2022multiface}
Nersemble~\cite{Kirschstein2023nersemble}
ActorsHQ~\cite{Icsik2023humanrf}
FFHQ~\cite{Karras2019style}
Goliath~\cite{Wuu2022multiface}
Ava-256~\cite{Martinez2024codec}
Facescape~\cite{Yang2020facescape, Zhu2023facescape}
MVHumanNet~\cite{Xiong2024mvhumannet}
OpenHumanVid~\cite{li2025openhumanvid}
David (Synthetic Dataset) ~\cite{Saleh2025david}
WildAvatar~\cite{huang2025wildavatar}


\VS{useful datasets for learning hair priors: USC-HairSalon, Hair20k, DiffLocks, Cem Yuksel's samples, CT2Hair, K-Hairstyle, for generation afro hair: Transforming Unstructured Hair Strands into Procedural Hair Grooms?~\cite{Chang2025transforming}}

==> tables/legend_names.tex <==
\begin{table*}[t]
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\textwidth}{@{} l X @{}}
\toprule
\multicolumn{2}{@{}l}{\textbf{Prior Stage}} \\
\midrule
Type         & \val{blue}{R}{Real} \valsep \val{orange}{S}{Synth} \valsep \val{purple}{G}{Generated} \\
Datasets     & \val{red}{I}{Internal} \valsep \val{teal}{V}{VFHQ} \valsep \val{violet}{F}{FFHQ} \valsep \val{brown}{H}{InterHand2.6M} \\
Modality     & \val{cyan}{S}{Single image} \valsep
                \val{lime}{C}{Mono video} \valsep
                \val{magenta}{V}{Multi-view video} \valsep
                \val{olive}{O}{OLAT multi-view video} \valsep
                \val{pink}{M}{Meshes} \valsep
                \val{yellow}{B}{MRI} \valsep
                \val{gray}{T}{3D Strands} \\
\midrule
\multicolumn{2}{@{}l}{\textbf{Creation Stage}} \\
\midrule
Inputs & \val{green}{Z}{Zero} \valsep
         \val{red}{N}{One} \valsep
         \val{blue}{F}{Few} \valsep
         \val{orange}{C}{Mono video} \valsep
         \val{purple}{V}{Multi-view video} \valsep
         \val{brown}{L}{OLAT multi-view video} \valsep
         \val{pink}{I}{Multi-view image} \valsep
         \val{gray}{D}{Depth} \valsep
         \val{cyan}{A}{Audio} \valsep
         \val{magenta}{U}{OLAT multi-view image} \valsep
         \val{yellow}{T}{Text \icoText} \\
Needed assets & \val{teal}{K}{Tracked 3DMM} \valsep \val{lime}{E}{Cameras} \valsep \val{violet}{Q}{Registered Meshes} \valsep \val{olive}{X}{Textures} \\
Speed        & \val{lightgray}{I}{Instant} \valsep
               \val{darkgray}{F}{Fast} \valsep
               \val{red!50}{M}{Medium} \valsep
               \val{blue!50}{S}{Slow} \\
\midrule
\multicolumn{2}{@{}l}{\textbf{Animation Stage}} \\
\midrule
Animation Signal & \val{blue}{D}{3DMM expr} \valsep
                   \val{orange}{G}{General expr} \valsep
                   \val{green}{A}{Audio audio} \valsep
                   \val{red}{V}{Video} \valsep
                   \val{purple}{T}{Text} \valsep
                   \val{brown}{P}{Pose} \valsep
                   \val{pink}{S}{Simulation} \\
Lighting & \val{cyan}{N}{None} \valsep
           \val{magenta}{L}{Local} \valsep
           \val{yellow}{D}{Distant} \\
Animation Speed & \val{teal}{R}{Real-time} \valsep
                  \val{lime}{I}{Interactive} \valsep
                  \val{violet}{O}{Offline} \\
\bottomrule
\end{tabularx}
\caption{Avatar pipeline taxonomy legend.}
\label{tab:avatar_pipeline_taxonomy}
\end{table*}
